Contextual Bandits with Side-Observations

We investigate contextual bandits in the presence of side-observations across arms in order to design recommendation algorithms for users connected via social networks. Users in social networks respond to their friends' activity, and hence provide information about each other's preferences. In our model, when a learning algorithm recommends an article to a user, not only does it observe his/her response (e.g. an ad click), but also the side-observations, i.e., the response of his neighbors if they were presented with the same article. We model these observation dependencies by a graph $\mathcal{G}$ in which nodes correspond to users, and edges correspond to social links. We derive a problem/instance-dependent lower-bound on the regret of any consistent algorithm. We propose an optimization (linear programming) based data-driven learning algorithm that utilizes the structure of $\mathcal{G}$ in order to make recommendations to users and show that it is asymptotically optimal, in the sense that its regret matches the lower-bound as the number of rounds $T\to\infty$. We show that this asymptotically optimal regret is upper-bounded as $O\left(|\chi(\mathcal{G})|\log T\right)$, where $|\chi(\mathcal{G})|$ is the domination number of $\mathcal{G}$. In contrast, a naive application of the existing learning algorithms results in $O\left(N\log T\right)$ regret, where $N$ is the number of users.

==> AISTATS Arxiv/discussion.tex <==
\section{Discussion}
In this paper we introduce a framework to incorporate side-observations into the contextual bandits with linear payoff functions. We derive an instance-dependent lower bound on the regret of any learning algorithm, and also an optimal algorithm whose regret matches these lower bounds asymptotically as $T\to\infty$. We plan to extend the results to the case when the set of arms to choose from is non-stationary.

==> AISTATS Arxiv/simul.tex <==
\section{Experiments}
\begin{figure}
\centering
\begin{subfigure}[b]{0.42\textwidth}
    \includegraphics[width=\textwidth]{Simulation/dim_2_numOfUsers_2_numOfArticles_5_er_1_1.pdf}
     \caption{$d = 2, N =2, K=5, p=1$}
     \label{fig:synthetic_1}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}
    \includegraphics[width=\textwidth]{Simulation/dim_4_numOfUsers_4_numOfArticles_10_er_05_1.pdf}
     \caption{$d = 4, N =4,K=10, p =0.5 $}
     \label{fig:synthetic_2}
\end{subfigure}
\label{fig:synthetic_numerical}
\begin{subfigure}[b]{0.42\textwidth}
    \includegraphics[width=\textwidth]{Simulation/dim_4_numOfUsers_10_numOfArticles_5_er_05.pdf}
     \caption{$d = 4, N =10,K=10, p =0.5 $}
     \label{fig:synthetic_3}
\end{subfigure}
\caption{Comparison of regret of Algorithm~\ref{algo:opt} with the algorithms  of~\cite{lattimore2016end}, which we denote as Lattimore and Lattimore-N. The plots are obtained after averaging the results of $100$ runs. $N$ and $K$ denote the number of users, and contexts respectively. The computational complexity of all the three algorithms is similar since they involve solving an optimization problem in which number of decision variables is equal to the number of arms.
}\label{fig:synthetic} % $p$ denotes the probability with which any two users are connected, and $d$ is the dimension of the context vector.
\end{figure}
\emph{Synthetic Data Experiment}: 
The vector $\theta=\left\{\theta\ust_i\right\}_{i\in \cV}$ that contains the coefficients of the users, and the contexts of the arms, are generated randomly; $\theta_i$, and the context vectors are drawn from a uniform distribution with support in the set $[0,1]^{d}$. The edges in the graph $\cG$ are drawn randomly; any two nodes $i,j\in\cV$ are connected with a probability $p$. The noise $\eta_{i}(t),\eta_{(i,j)}(t)$ associated with the rewards and the side-observations~\eqref{def:reward},~\eqref{def:side_obs} are assumed to be Gaussian with standard deviation $0.1$. We compare the performance of Algorithm~\ref{algo:opt} with the algorithm of~\cite{lattimore2016end}, which is denoted Lattimore, and its adapation to the graphical setting which is denoted Lattimore-N. Lattimore-N is a naive adaptation of Lattimore algorithm, it uses side observations to enhance the estimation after warm-up phase, our experimental results show the potential gains from using the side observations alone. However, by leveraging the graph structure, our optimal algorithm shows significant regret reduction, and verifies our theoretical claims. We summarize the results of this evaluation in Figure~\ref{fig:synthetic}, where we plot the cumulative regret
of the algorithms as a function of rounds, averaged over $100$ runs.

%dim_2_numOfUsers_2_numOfArticles_5_er_1

==> discussion.tex <==
\section{Discussion}
In this paper we introduce a framework to incorporate side-observations into the contextual bandits with linear payoff functions. We derive an instance-dependent lower bound on the regret of any learning algorithm, and also an optimal algorithm whose regret matches these lower bounds asymptotically as $T\to\infty$. We plan to extend the results to the case when the set of arms to choose from is non-stationary.

==> simul.tex <==
\section{Experiments}
\begin{figure}
\centering
\begin{subfigure}[b]{0.42\textwidth}
    \includegraphics[width=\textwidth]{Simulation/dim_2_numOfUsers_2_numOfArticles_5_er_1_1.pdf}
     \caption{$d = 2, N =2, K=5, p=1$}
     \label{fig:synthetic_1}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}
    \includegraphics[width=\textwidth]{Simulation/dim_4_numOfUsers_4_numOfArticles_10_er_05_1.pdf}
     \caption{$d = 4, N =4,K=10, p =0.5 $}
     \label{fig:synthetic_2}
\end{subfigure}
\label{fig:synthetic_numerical}
\begin{subfigure}[b]{0.42\textwidth}
    \includegraphics[width=\textwidth]{Simulation/dim_4_numOfUsers_10_numOfArticles_5_er_05.pdf}
     \caption{$d = 4, N =10,K=10, p =0.5 $}
     \label{fig:synthetic_3}
\end{subfigure}
\caption{Comparison of regret of Algorithm~\ref{algo:opt} with the algorithms  of~\cite{lattimore2016end}, which we denote as Lattimore and Lattimore-N. The plots are obtained after averaging the results of $100$ runs. $N$ and $K$ denote the number of users, and contexts respectively. The computational complexity of all the three algorithms is similar since they involve solving an optimization problem in which number of decision variables is equal to the number of arms.
}\label{fig:synthetic} % $p$ denotes the probability with which any two users are connected, and $d$ is the dimension of the context vector.
\end{figure}
\emph{Synthetic Data Experiment}: 
The vector $\theta=\left\{\theta\ust_i\right\}_{i\in \cV}$ that contains the coefficients of the users, and the contexts of the arms, are generated randomly; $\theta_i$, and the context vectors are drawn from a uniform distribution with support in the set $[0,1]^{d}$. The edges in the graph $\cG$ are drawn randomly; any two nodes $i,j\in\cV$ are connected with a probability $p$. The noise $\eta_{i}(t),\eta_{(i,j)}(t)$ associated with the rewards and the side-observations~\eqref{def:reward},~\eqref{def:side_obs} are assumed to be Gaussian with standard deviation $0.1$. We compare the performance of Algorithm~\ref{algo:opt} with the algorithm of~\cite{lattimore2016end}, which is denoted Lattimore, and its adapation to the graphical setting which is denoted Lattimore-N. Lattimore-N is a naive adaptation of Lattimore algorithm, it uses side observations to enhance the estimation after warm-up phase, our experimental results show the potential gains from using the side observations alone. However, by leveraging the graph structure, our optimal algorithm shows significant regret reduction, and verifies our theoretical claims. We summarize the results of this evaluation in Figure~\ref{fig:synthetic}, where we plot the cumulative regret
of the algorithms as a function of rounds, averaged over $100$ runs.

%dim_2_numOfUsers_2_numOfArticles_5_er_1
